Can We Count on LLMs? The Fixed-Effect Fallacy and Claims of GPT-4 Capabilities

In this paper we explore evaluation of LLM capabilities. We present measurements of GPT-4 performance on several deterministic tasks; each task involves a basic calculation and takes as input parameter some element drawn from a large well-defined population (e.g., count elements in a list, multiply two k-digit numbers, etc). We examine several conditions per-task and perform enough trials so that statistically significant differences can be detected. This allows us to investigate the sensitivity of task-accuracy both to query phrasing and input parameter population. We find that seemingly trivial modifications in the task-prompt or input population can yield differences far larger than can be explained by sampling effects. For example, performance on a simple list-counting task varies with query-phrasing and list-length, but also with list composition (i.e., the thing-to-be-counted) and object frequency (e.g., success when an element accounts for $\approx$ 50\% of a list is different from when it accounts for $\approx$ 70\% etc). We conclude that efforts to quantify LLM capabilities easily succumb to the language-as-fixed-effect fallacy, where experimental observations are improperly generalized beyond what the data supports. A consequence appears to be that intuitions that have been formed based on interactions with humans form a very unreliable guide as to which input modifications should ``make no difference'' to LLM performance.

==> listQueries/composite.tex <==
\subsection{Composite Query}
\label{sec:composite}

Finally we examine performance on a composite query; e.g.,  evaluate performance on tasks that consists of sub-tasks A, B, and C and compare the resulting performance with the product of the performance on the sub-tasks. We will use the already-evaluated tasks from earlier sections as our sub-tasks. An example query is:

\chatPrompt{``Find the maximum and median of this list, and then calculate their product: [24, 85, 12, 67, 55, 88, 51, 11, 66, 47, 45]. Please write `Answer='''}{4488}{4840}

For a length $N=11$ list our measured value with $500$ trials of this query was correct $79.0$\% of the time. 
Using GPT-4 with a list of N=11 integers drawn from $(10, 99)$ the maximum and median are correct 99.9\% and 89.6\%
of the time respectively (these can be found from Column 3 of Tables \ref{tab:maxTable} and \ref{tab:medianTable}
respectively. The product for 2-digit by 2-digit is correct 100.0\% of the time (as shown in Table \ref{tab:multiply}).
Collectively, these imply that the product of maximum and median should be correct $0.999 \times 0.896 \times 1.0$ or
$89.5$\% of the time.   

We repeat this analysis for the other lengths.
For the length $N=15$ list our measured value was correct $69.8$\% of the time, versus and expected $79.9$\%.
For the length $N=21$ list our measured value was correct  $57.4$\% of the time, versus and expected  $63.6$\%.

In each case we again have a gap between observed and expected that is larger than  can be explained by a 
traditional estimate of margin-of-error. That performance on composite tasks is often lower than the product
of the performance on sub-tasks is also observed by Dziri et al \citep{dziri2023faith}.
 



% Using GPT-3.5: the product of median and maximum is correct $62.9 \pm 5.7$\%. However, the median is correct $79.1 \pm 2.4$\% of the time and the maximum and 2-digit product are correct  $> 99$\%
% of the time. Thus the composite accuracy of the task appears lower than the product of the individual accuracies. 



==> listQueries/effects.tex <==
\section{Working list of observations}

\begin{enumerate}
\item Counting (and max, median, sort etc) is hard. Eg, Table I. Performance decreases significantly with list-size.
\item Answers seem significantly \btr, and biased (eg, under-counting more common than over-counting see after Table \ref{tab:count}).
\item GPT-3.5 follows same trends (see Section \ref{sec:gpt35}). GPT-3.5 is usually worse, but sometimes better (see count Distinct Table \ref{tab:countDistinct})
\item The inputs matter. Compare the columns in Table I (statistically significant differences).
\item Rewording matters: Table \ref{tab:count35}
\item Name-value lists have different behavior to value lists. Table \ref{tab:aggreg20k} versus Table \ref{tab:nameValue20k} (Median is worse for value as opposed to name-value, sort is better)
\item Max, Median and Sort
\begin{itemize}
\item \# decimal places doesn't seem important. Eg, Table \ref{tab:aggreg20k} versus Table \ref{tab:aggreg20k_12sigFigs}
\item Leading digits maybe important? Eg, Table \ref{tab:aggreg20k} versus Table \ref{tab:aggregSamePrefix} 
\end{itemize}
\item Long-multiply:
\begin{itemize}
\item Asymmetric: $2 \times 5$ etc has better performance than $5 \times 2$ ? Table \ref{tab:multiply} and Table \ref{tab:multiply35}
\item The answers seem considerable \btr 
\item Surface probabilities appear to matter a lot: first, last digits mostly correct.
\end{itemize}
\end{enumerate}
%
%\begin{itemize}
%\item Generalizing that seemingly irrelevant changes make no difference is really tricky. 
%\item When can we generalize from an observation? Instead of `logically equivalent' seems we need top consider `probabilities don't change'
%\end{itemize}


==> listQueries/gpt3.5 <==
\section{GPT-3.5-turbo stuff}

\begin{table}[h]
\center{
\begin{tabular}{ccccc}\hline
$N$ &   mango/peach & airedale/aspidistra & xhsfgre/jnosdfi\\ \hline  
%$10$ & 75.6 $\pm$ 3.76\% &68.6 $\pm$ 4.07\% &68.2 $\pm$ 4.08\% &\\ \hline
%$15$ & 26.8 $\pm$ 3.88\% &32.0 $\pm$ 4.09\% &33.2 $\pm$ 4.13\% &\\ \hline
%$20$ & 13.8 $\pm$ 3.02\% &8.2 $\pm$ 2.4\% &7.8 $\pm$ 2.35\% &\\ \hline
%
$10$ & 75.6\% &68.6\% &68.2\% &\\ \hline
$15$ & 26.8\% &32.0\% &33.2\% &\\ \hline
$20$ & 13.8\% &8.2\% &7.8\% &\\ \hline
$30$ & 12.2\% &5.0\% &4.0\% &\\ \hline
$40$ & 7.8\% &2.2\% &1.2\% &\\ \hline
%100 & & 0\% & & \\ \hline 
\end{tabular}
}
\caption{\label{tab:count} GPT-3.5-turbo: Percent correct for counting  the occurrences of a length-$N$ list with two items chosen uniformly at random.}
\end{table}

The performance of GPT-3.5-turbo is worse than GPT-4, but follow the pattern that mango/peach is an easier task than airedale/aspidistra and that the later has 
similar performance to two random strings.


==> listQueries/gpt35.tex <==
\section{GPT-3.5-turbo stuff}
\label{sec:gpt35}
\begin{table}[h]
\center{
\begin{tabular}{ccccc}\hline
$N$  & \shortstack{mango/\\peach} & \shortstack{airedale/\\aspidistra} & \shortstack{xhsfgre/\\jnosdfi} & Reworded \\ \hline
%$N$ &   mango/peach & airedale/aspidistra & xhsfgre/jnosdfi  & Reworded \\ \hline  
%$10$ & 75.6 $\pm$ 3.76\% &68.6 $\pm$ 4.07\% &68.2 $\pm$ 4.08\% &\\ \hline
%$15$ & 26.8 $\pm$ 3.88\% &32.0 $\pm$ 4.09\% &33.2 $\pm$ 4.13\% &\\ \hline
%$20$ & 13.8 $\pm$ 3.02\% &8.2 $\pm$ 2.4\% &7.8 $\pm$ 2.35\% &\\ \hline
%
$10$ & 75.6\% &68.6\% &68.2\% & 89.4\%\\ \hline
$15$ & 26.8\% &32.0\% &33.2\% & 55.6\% \\ \hline
$20$ & 13.8\% &8.2\% &7.8\% & 33.0\% \\ \hline
$30$ & 12.2\% &5.0\% &4.0\% & 13.8\% \\ \hline
$40$ & 7.8\% &2.2\% &1.2\% & 8.8\% \\ \hline
%100 & & 0\% & & \\ \hline 
\end{tabular}
}
\caption{\label{tab:count35} GPT-3.5-turbo: Percent correct for counting  the occurrences of a length-$N$ list with two items chosen uniformly at random.}
\end{table}

The performance of GPT-3.5-turbo is worse than GPT-4, but follow the pattern that mango/peach is an easier task than airedale/aspidistra and that the later has 
similar performance to two random strings.


\begin{table}[h]
\center{
\begin{tabular}{cccc}\hline
  & Max. & Median & Sort \\ \hline
11   & 100\% & 84.8\% & 99.7\%\\ \hline
15  & 100\%  & 74.0\% & 98.0\%  \\ \hline
21   & 97\% & 62.7\% & 99.7\% \\ \hline 
%31   & & \\ \hline
%51 & & 25\% &  \\ \hline
%101 & & & 0\% \\ \hline 
\end{tabular}
}
\caption{\label{tab:count2sigit_35} GPT-3.5-turbo: Percent correct for Min, Max, Median and Sort of a length-$N$ list of two-digit integers.  Integers were uniformly distributed on $(10, 99).$}
\end{table}


\begin{table}[h]
\center{
\begin{tabular}{cccc}\hline
  & Max. & Median & Sort \\ \hline
11   & 96.0\% & 44.2\% & 13.2\%\\ \hline
15  & 93.8\%  & 18.2\% & 2.2\% \\ \hline
21  & 88.6\% & 6.8\% & 0\%\\ \hline 
%31   & & \\ \hline
%51 & & 25\% &  \\ \hline
%101 & & & 0\% \\ \hline 
\end{tabular}
}
\caption{\label{tab:nameValue20k_gpt35} GPT-3.5-turbo: Percent correct for Min, Max, Median and Sort of  a list of $N$ name-value pairs. Numbers were uniformly distributed on $(100.0, 20000.0).$}
\end{table} 

\begin{table}[h]
\center{
\begin{tabular}{ccccc}\hline
\diaghead(-3,2){.1em}{$k_1$}{$k_2$} & 2 & 3 & 4 & 5 \\ \hline
% $2$ & 100.0 $\pm$ 4.34\% &57.0 $\pm$ 4.34\% &38.4 $\pm$ 4.26\%  \\ \hline
% $3$ & 71.0 $\pm$ 3.98\% &40.8 $\pm$ 4.31\% &5.6 $\pm$ 2.02\%  \\ \hline
% $4$ & 50.4 $\pm$ 4.38\% &11.4 $\pm$ 2.79\% &0.5 $\pm$ 0.69\%  \\ \hline
  $2$ & 100.0\% &57.0\% &38.4\% & 19.0\% \\ \hline
 $3$ & 71.0\% &40.8 \% &5.6\%  \\ \hline
 $4$ & 50.4 \% &11.4 \% &0.5\%  \\ \hline
 $5$ & 25.8\% & 3.4\% & \\ \hline
\end{tabular}
}
\caption{\label{tab:multiply35} GPT-3.5-turbo: Percent correct for multiplying a $k_1$-digit by $k_2$-digit number.}
\end{table}


==> listQueries/theories.tex <==
\section{What's going on?}

\subsection{Observations}
\label{sec:observations}
\begin{itemize}
\item This is a failure mode quite distinct from hallucinations
\item At a certain size we seem to be always wrong
\item Answers are significantly \btr
\item Surface probabilities are often(?) learned: first/last digits of multiply, comma versus other separator, 
\item Problem occurs at much smaller than \# attention heads.
\end{itemize}



\subsection{Limits of Autoregression}

More common output sequences are more likely to be chosen.  $\max P(\mbox{Output}|\mbox{Input)} \propto \max P(\mbox{Input}|\mbox{Output)}  \cdot P(\mbox{Output)}.$

In answer to the objection that maybe CoT or similar would allow the model to get some of these queries right: ``That is, our core predictions are of the form `for LLMs, X is harder than Y' rather than `LLMs can’t do X.'''
\cite{mccoy2023embers}
Thus, the fact that accuracy is a function of prompt phrasing is already an indication that the task is harder for the model than tasks where phrasing doesn't matter.

Impact of pre-training term frequencies \cite{razeghi2022impact}. Time-unit conversion, celsius-to-fahrenheit etc.
\subsection{Limits of Attention} 

Attention tells the model which tokens in the context window are most helpful in predicting the next token \cite{vaswani2017attention}. Explanations of what exactly it does are a bit hand-wavey. Several of the tasks we give in Section \ref{sec:tasks}
require paying attention to every element in a list. That is, one can't ignore any token in a list and still be sure that counting, sorting, max, etc will be done correctly. Thus at some point we might just overload the 
number of attention heads. Interestingly, failure starts to happen at much lower numbers than the number of attention heads.

There are $Q^N$ length-$N$ lists of $Q$ items. Choosing them uniformly-at-random explicitly breaks the assumption that some sequences are a lot more likely than others.

Are limits of autoregression, attention related? 

\subsection{Reasons for Optimism}
Better-than-random offers hope. The fact that there's a bias to the answers (e.g., usually under-counting by 1) is indicative of bias rather than variance.
Improvement from GPT-3.5 is encouraging.



% \subsection{Locate}

% Locate the $k$-th element in a set. 
% \begin{itemize}
% \item Letter in string
% \item Digit in number
% \item Word in sentence
% \item ``What is the third sentence of A Tale of Two Cities?''
% \end{itemize}

% \subsection{Other things it gets wrong}
% \begin{itemize}
% \item Write a poem but use ABAB rhyme-scheme (any poetry output seems dominated by 8-syllable rhyming couplets).
% \item Basic calculations in roman numerals

% \end{itemize} 

==> listQueries/todo.tex <==
\section{To do} 

\begin{itemize}
\item Gather comprehensive stats for each of the list queries. Nice display format for example queries/asnwers (eg, format in \cite{mccoy2023embers} is nice).
\item Other models, eg, PaLM, Llama.
\item What's a good measure of how close answer is to correct; eg, sorting, location (out-of-list errors)
\item What's the best tap-in point for n\_head, n\_layer LLM to explore attention? Feature engineering over the attention outputs?
\item Can we tell anything from $P(\mbox{Output)}$ being high? Ie, no access to weights?
\item Are the trends that appear in gpt-35 also there in gpt-4?
\end{itemize} 
